SQ Lower Bounds for Random Sparse Planted Vector Problem

Consider the setting where a $\rho$-sparse Rademacher vector is planted in a random $d$-dimensional subspace of $R^n$. A classical question is how to recover this planted vector given a random basis in this subspace. A recent result by [ZSWB21] showed that the Lattice basis reduction algorithm can recover the planted vector when $n\geq d+1$. Although the algorithm is not expected to tolerate inverse polynomial amount of noise, it is surprising because it was previously shown that recovery cannot be achieved by low degree polynomials when $n\ll \rho^2 d^{2}$ [MW21]. A natural question is whether we can derive an Statistical Query (SQ) lower bound matching the previous low degree lower bound in [MW21]. This will - imply that the SQ lower bound can be surpassed by lattice based algorithms; - predict the computational hardness when the planted vector is perturbed by inverse polynomial amount of noise. In this paper, we prove such an SQ lower bound. In particular, we show that super-polynomial number of VSTAT queries is needed to solve the easier statistical testing problem when $n\ll \rho^2 d^{2}$ and $\rho\gg \frac{1}{\sqrt{d}}$. The most notable technique we used to derive the SQ lower bound is the almost equivalence relationship between SQ lower bound and low degree lower bound [BBH+20, MW21].

==> content/InfoLowerBound.tex <==
\section{Information Theoretic Lower Bound}

In this section, we prove the information theoretic lower bound in theorem \ref{theorem_infolb1} and theorem \ref{theorem_infolb2} using Le Cam's Contiguity \cite{kunisky2019notes}.

\subsection{Likelihood Ratio}

In the setting of problem \ref{problem_detection}, we have:
\begin{itemize}
	\item Null distribution $\cQ$: observe $\tilde{Z} \in \R^{n \times d}$ whose entries are i.i.d. sampled from standard Gaussian $N(0, 1)$. Therefore, distribution $\cQ$ is the product of $n$ standard Gaussian $N(0,\Id_d)^{\otimes n}$.
	\item Planted distribution $\cP$: observe $\tilde{Z}$ according to model \ref{model_general}. Therefore, distribution $\cP$ is $\otimes_{i \in [n]} N(x_i u, \Sigma_u)$ where $x_i$ are i.i.d. Bernoulli-Rademacher entries, $u \sim S^{d-1}$ is uniformly drawn from the unit sphere and $\Sigma_u = \Id_d - u u^{\top} + \sigma^2 u u^{\top}$.
\end{itemize}
For simplicity, let us denote the probability density of $\cQ$ and $\cP$ as $\mu_0$ and $\mu_1$ respectively, i.e. $\mu_0(Z) = d \cQ (Z)$ and $\mu_1(Z) = d \cP (Z)$. Denote the likelihood ratio by $L(Z) = \frac{d \cP}{d \cQ} (Z) = \frac{\mu_1(Z)}{\mu_0(Z)}$. The goal is to show that the second moment of likelihood ratio $E_{Z \sim \mu_0} [(L(Z))^2]$ remains bounded as $d \rightarrow \infty$, i.e. to prove the following theorem.

\subsection{From Multiple Sample to Single Sample}

In the following sections, we write $\bar{D}_{u, x_u} (z) = \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)}$, where $D_{u, x_u}(z)$ is the probability that sample $z$ is drawn from $N(x_u u, \Sigma_u)$ and $D_{\emptyset}(z)$ is the probability that sample $z$ is drawn from $N(0, \Id_d)$. The following proposition allows us to simplify the computation of multiple-sample likelihood ratio by reducing it to computation of single-sample likelihood ratio and focusing on computing $\E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]$.

\begin{proposition}
\label{prop_multiSampleToSingleSample}
For $L(Z) = \frac{\mu_1(Z)}{\mu_0(Z)}$ and $\bar{D}_{u, x_u} (z) = \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)}$,
\begin{equation}
\label{eq_multisample}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = \E_{u, v \sim S^{d-1}} \Brac{ \Paren{\E_{x_u, x_v}\Brac{\E_{z \sim D_{\emptyset}}\Brac{\iprod{\bar{D}_{u, x_u} (z),\bar{D}_{v, x_v} (z)}}}}^n}
\end{equation}
\end{proposition}

\begin{proof}
    From the definition of likelihood ratio, we have:
    \begin{align*}
        L(Z) & = \frac{\mu_1(Z)}{\mu_0(Z)} \\
        & = \frac{\E_{u, x_1, x_2, \dots, x_{n}}[\Pi_{i=1}^{n} D_{u, x_i} (z_i)]}{\Pi_{i=1}^{n} D_{\emptyset}(z_i)} \\
        & = \E_{u, x_1, x_2, \dots, x_{n}}[\Pi_{i=1}^{n} \bar{D}_{u, x_i} (z_i)] \\
        & = \E_{u \sim S^{d-1}}[\Pi_{i=1}^{n} \E_{x_i}[\bar{D}_{u, x_i} (z_i)]]
    \end{align*}
    Plug this into $\E_{Z \sim \mu_0} [(L(Z))^2]$, we get:
    \begin{align*}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        & = \E_{Z \sim \mu_0} \Brac{\Paren{\E_{u \sim S^{d-1}}[\Pi_{i=1}^{n} \E_{x_i}[\bar{D}_{u, x_i} (z_i)]]}^2} \\
        & = \E_{Z \sim \mu_0} \Brac{\E_{u \sim S^{d-1}}[\Pi_{i=1}^{n} \E_{x_{u, i}}[\bar{D}_{u, x_{u, i}} (z_i)]] \cdot \E_{v \sim S^{d-1}}[\Pi_{i=1}^{n} \E_{x_{v,i}}[\bar{D}_{v, x_{v,i}} (z_i)]]} \\
        & = \E_{Z \sim \mu_0} \Brac{\E_{u, v \sim S^{d-1}}[\Pi_{i=1}^{n} \big( \E_{x_{u, i}}[\bar{D}_{u, x_{u, i}} (z_i)] \cdot \E_{x_{v,i}}[\bar{D}_{v, x_{v,i}} (z_i)] \big)]} \\
        & = \E_{u, v \sim S^{d-1}} \Brac{\Pi_{i=1}^{n} \E_{z_i \sim D_{\emptyset}}[\E_{x_{u, i}}[\bar{D}_{u, x_{u, i}} (z_i)] \cdot \E_{x_{v, i}}[\bar{D}_{v, x_{v, i}} (z_i)]]} \\
        & = \E_{u, v \sim S^{d-1}} \Brac{ \Paren{\E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]}^n}
    \end{align*}
    where the last step is because $\E_{z_i \sim D_{\emptyset}}[\E_{x_{u, i}}[\bar{D}_{u, x_{u, i}} (z_i)] \cdot \E_{x_{v, i}}[\bar{D}_{v, x_{v, i}} (z_i)]] = \E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]$ is the same for all $i$.
\end{proof}

\subsection{Single Sample}

We first focus on computing $\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]$, as computing expectation over $x_u, x_v$ is fairly straightforward.

\begin{proposition}
\label{prop_singelSampleEz}
Let $\theta = 1- \sigma^2$ and $c = u^{\top} v$. For $\bar{D}_{u, x_u} (z) = \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)}$ and $\bar{D}_{v, x_v} (z) = \frac{D_{v, x_v} (z)}{D_{\emptyset}(z)}$,
\begin{equation}
    \label{eq_singlesampleEz}
    \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
    = \frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}}
\end{equation}
\end{proposition}

\begin{proof}
    Since $\bar{D}_{u, x_u} (z) = \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)}$, we have:
    \begin{align}
    \label{eq_singlesample1}
    \begin{split}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        & = \int_z \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)} \cdot \frac{D_{u, x_u} (z)}{D_{\emptyset}(z)} D_{\emptyset}(z) dz \\
        & = \int_z \frac{\exp(-\frac{1}{2} \Delta)}{\sqrt{(2 \pi)^d |\Sigma_u| |\Sigma_v|}} dz
    \end{split}
    \end{align}
    where $\Delta = (z- x_u u)^{\top} \Sigma_u^{-1}(z- x_u u) + (z- x_v v)^{\top} \Sigma_v^{-1}(z- x_v v) - z^{\top} \Id_d^{-1} z$. Since $\Sigma_u^{-1} = \Id_d - u u^{\top} + \frac{1}{\sigma^2} u u^{\top}$ and $\Sigma_v^{-1} = \Id_d - v v^{\top} + \frac{1}{\sigma^2} v v^{\top}$, we have:
    \begin{align*}
        \Delta
        & = (z- x_u u)^{\top} \Sigma_u^{-1}(z- x_u u) + (z- x_v v)^{\top} \Sigma_v^{-1}(z- x_v v) - z^{\top} \Id_d^{-1} z \\
        & = z^{\top} (\Sigma_u^{-1} + \Sigma_v^{-1} - \Id_d) z - 2 x_u z^{\top}\Sigma_u^{-1} u -  2 x_v z^{\top}\Sigma_v^{-1} v + x_u^2 u^{\top}\Sigma_u^{-1} u + x_v^2 v^{\top}\Sigma_v^{-1} v \\
        & = z^{\top} (\Sigma_u^{-1} + \Sigma_v^{-1} - \Id_d) z - \frac{2 x_u}{\sigma^2} z^{\top} u -  \frac{2 x_v}{\sigma^2} z^{\top} v + \frac{x_u^2}{\sigma^2} + \frac{x_v^2}{\sigma^2} \\
        & = z^{\top} (\Sigma_u^{-1} + \Sigma_v^{-1} - \Id_d) z - \frac{2}{\sigma^2} (x_u u + x_v v)^{\top} z + \frac{1}{\sigma^2} (x_u^2 + x_v^2)
    \end{align*}
    Let $M = \Sigma_u^{-1} + \Sigma_v^{-1} - \Id_d$, we have:
    \begin{align*}
        \Delta
        = & z^{\top} M z - \frac{2}{\sigma^2} (x_u u + x_v v)^{\top} z + \frac{1}{\sigma^2} (x_u^2 + x_v^2) \\
        = & (z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v))^{\top}M(z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v)) - \frac{1}{\sigma^4} (x_u u + x_v v)^{\top} M^{-1} (x_u u + x_v v) \\
        & + \frac{1}{\sigma^2} (x_u^2 + x_v^2)
    \end{align*}
    Plug this into equation \ref{eq_singlesample1}, we get:
    \begin{align*}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        & = \int_z \frac{\exp(-\frac{1}{2} \Delta)}{\sqrt{(2 \pi)^n |\Sigma_u| |\Sigma_v|}} dz \\
        & = \int_z \frac{\exp(-\frac{1}{2} (z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v))^{\top}M(z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v)))\cdot \exp(W)}{\sqrt{(2 \pi)^n |\Sigma_u| |\Sigma_v|}} dz \\
        & = \frac{\exp(W)}{\sqrt{|\Sigma_u| |\Sigma_v| |M|}} \int_z \frac{\exp(-\frac{1}{2} (z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v))^{\top}M(z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v)))}{\sqrt{(2 \pi)^n |M^{-1}|}} dz
    \end{align*}
    where $W = \frac{1}{2\sigma^4} (x_u u + x_v v)^{\top} M^{-1} (x_u u + x_v v) - \frac{1}{2\sigma^2} (x_u^2 + x_v^2)$. Notice that $ \frac{\exp(-\frac{1}{2} (z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v))^{\top}M(z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v)))}{\sqrt{(2 \pi)^n |M^{-1}|}}$ is the probability density function of Gaussian distribution $N(\frac{M^{-1}}{\sigma^2}(x_u u + x_v v), M^{-1})$. Therefore,
    \begin{equation*}
        \int_z \frac{\exp(-\frac{1}{2} (z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v))^{\top}M(z - \frac{M^{-1}}{\sigma^2}(x_u u + x_v v)))}{\sqrt{(2 \pi)^n |M^{-1}|}} dz = 1
    \end{equation*}
    and, plug this into $\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]$, we get:
    \begin{equation}
    \label{eq_singlesample2}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        = \frac{\exp(W)}{\sqrt{|\Sigma_u| |\Sigma_v| |M|}}
    \end{equation}
    Now, consider $M = \Sigma_u^{-1} + \Sigma_v^{-1} - \Id_d$. Plug in $\Sigma_u^{-1} = \Id_d - u u^{\top} + \frac{1}{\sigma^2} u u^{\top}$ and $\Sigma_v^{-1} = \Id_d - v v^{\top} + \frac{1}{\sigma^2} v v^{\top}$, we get:
    \begin{align*}
        M
        & = \Id_d + (\frac{1}{\sigma^2} - 1) u u^{\top} + (\frac{1}{\sigma^2} - 1) v v^{\top} \\
        & = \Id_d + \alpha^2 C C^{\top}
    \end{align*}
    where $\alpha = \sqrt{\frac{1}{\sigma^2} - 1}$ and $C = [u, v]$ is the matrix whose two columns are $u$ and $v$. By the Woodbury Matrix Identity, we can compute $M^{-1}$ as:
    \begin{align*}
        M^{-1}
        & = (\Id_d + \alpha^2 C C^{\top})^{-1} \\
        & = \Id_d - \alpha^2 C(\Id_2 + \alpha^2 C^{\top} C)^{-1} C^{\top}
    \end{align*}
    Since
    $C^{\top} C =
    \begin{bmatrix}
    1 & u^{\top}v \\
    u^{\top}v & 1
    \end{bmatrix}$,
    we have:
    \begin{equation*}
        \Id_2 + \alpha^2 C^{\top} C
        = \Id_2 + (\frac{1}{\sigma^2} - 1) \begin{bmatrix} 1 & u^{\top}v \\ u^{\top}v & 1 \end{bmatrix}
        = \begin{bmatrix} \frac{1}{\sigma^2} & (\frac{1}{\sigma^2} - 1) u^{\top}v \\ (\frac{1}{\sigma^2} - 1) u^{\top}v & \frac{1}{\sigma^2} \end{bmatrix}
    \end{equation*}
    Take the inverse of this matrix, we get:
    \begin{equation*}
        (\Id_2 + \alpha^2 C^{\top} C)^{-1}
        = \frac{1}{1-(1 - \sigma^2)^2(u^{\top} v)^2}
        \begin{bmatrix} \sigma^2 & (\sigma^4 - \sigma^2) u^{\top}v \\ (\sigma^4 - \sigma^2) u^{\top}v & \sigma^2 \end{bmatrix}
    \end{equation*}
    Plug this into $M^{-1}$, we get:
    \begin{equation*}
        M^{-1} = \Id_d - \frac{1 / \sigma^2 -1}{1 - (1 - \sigma^2)^2(u^{\top} v)^2}
        C \begin{bmatrix} \sigma^2 & (\sigma^4 - \sigma^2) u^{\top}v \\ (\sigma^4 - \sigma^2) u^{\top}v & \sigma^2 \end{bmatrix} C^{\top}
    \end{equation*}
    Plug in $C = [u, v]$, we get:
    \begin{align*}
        M^{-1}
        & = \Id_d - \frac{1 / \sigma^2 - 1}{1 - (1 - \sigma^2)^2 (u^{\top} v)^2}
        [\sigma^2 u u^{\top} + \sigma^2 v v^{\top} + (\sigma^4 - \sigma^2) u^{\top} v v u^{\top} + (\sigma^4 - \sigma^2) u^{\top} v u v^{\top}] \\
        & = \Id_d - \frac{1 - \sigma^2}{1 - (1 - \sigma^2)^2 (u^{\top} v)^2}
        [u u^{\top} + v v^{\top} + (\sigma^2 - 1) u^{\top} v v u^{\top} + (\sigma^2 - 1) u^{\top} v u v^{\top}]
    \end{align*}
    Plug in $c = u^{\top} v$ and we have:
    \begin{equation*}
        M^{-1}
        = \Id_d - \frac{1 - \sigma^2 }{1 - (1 - \sigma^2)^2 c^2}
        [u u^{\top} + v v^{\top} + (\sigma^2 - 1) c v u^{\top} + (\sigma^2 - 1) c u v^{\top}]
    \end{equation*}
    Plug $M^{-1}$ into the expression of $W$, we get:
    \begin{align*}
        W
        = & \frac{1}{2\sigma^4} (x_u u + x_v v)^{\top} M^{-1} (x_u u + x_v v) - \frac{1}{2\sigma^2} (x_u^2 + x_v^2) \\
        = & \frac{1}{2\sigma^4} (x_u u + x_v v)^{\top} \Id_d (x_u u + x_v v) - \frac{1}{2\sigma^2} (x_u^2 + x_v^2) \\
        & - \frac{1}{2\sigma^4} \frac{1 - \sigma^2}{1 - (1 - \sigma^2)^2 c^2} (x_u u + x_v v)^{\top}
        [u u^{\top} + v v^{\top} + (\sigma^2 - 1) c v u^{\top} + (\sigma^2 - 1) c u v^{\top}] (x_u u + x_v v) \\
        = & (\frac{1}{2\sigma^4} - \frac{1}{2\sigma^2}) (x_u^2 + x_v^2) + \frac{x_u x_v c}{\sigma^4} \\
        & - \frac{1}{2\sigma^4} \frac{1 - \sigma^2}{1 - (1 - \sigma^2)^2  c^2} [(x_u^2 + x_v^2) + 2(\sigma^2+1)x_u x_v c + (2 \sigma^2 - 1)(x_u^2+ x_v^2)c^2 + 2(\sigma^2-1)x_u x_v c^3] \\
        = & \frac{1}{2 - 2 (1 - \sigma^2)^2 c^2} [2 x_u x_v c - (1 - \sigma^2)(x_u^2 + x_v^2)c^2]
    \end{align*}
    Plug this into equation \ref{eq_singlesample2}, we get:
    \begin{equation*}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        = \frac{\exp \Paren{\frac{1}{2 - 2 (1 - \sigma^2)^2 c^2} [2 x_u x_v c - (1 - \sigma^2)(x_u^2 + x_v^2)c^2]}}{\sqrt{|\Sigma_u| |\Sigma_v| |M|}}
    \end{equation*}
    Next, we compute $|\Sigma_u|$, $|\Sigma_v|$ and $|M|$. Since $\Sigma_u = \Id_d - u u^{\top} + \sigma^2 u u^{\top}$ and $\Sigma_v = \Id_d - v v^{\top} + \sigma^2 v v^{\top}$, we know that $\Sigma_u$ and $\Sigma_v$ has eigenvalue $\sigma^2$ with corresponding eigenvectors $u$ and $v$ respectively, and the rest of the eigenvalues are all 1's. Therefore, we have $|\Sigma_u| = \sigma^2$ and $|\Sigma_v| = \sigma^2$. Regarding $|M|$, we have $M = \Id_d + \alpha^2 C C^{\top}$ where $\alpha = \sqrt{\frac{1}{\sigma^2} - 1}$ and $C = [u, v]$. By the Matrix Determinant Lemma, we have:
    \begin{equation*}
        |M| = |\Id_d + \alpha^2 C C^{\top}|
        = |\Id_2 + \alpha^2 C^{\top} C|
        = |\begin{bmatrix} \frac{1}{\sigma^2} & (\frac{1}{\sigma^2} - 1) u^{\top}v \\ (\frac{1}{\sigma^2} - 1) u^{\top}v & \frac{1}{\sigma^2} \end{bmatrix}|
        = \frac{1}{\sigma^4} - (\frac{1}{\sigma^2} - 1)^2 c^2
    \end{equation*}
    Therefore,
    \begin{equation*}
        |\Sigma_u| |\Sigma_v| |M|
        = \sigma^2 \cdot \sigma^2 \cdot (\frac{1}{\sigma^4} - (\frac{1}{\sigma^2} - 1)^2 c^2)
        = 1 - (1 - \sigma^2)^2 c^2
    \end{equation*}
    Plug this into equation \ref{eq_singlesample2}, we get:
    \begin{equation*}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        = \frac{\exp \Paren{\frac{1}{2 - 2 (1 - \sigma^2)^2 c^2} [2 x_u x_v c - (1 - \sigma^2)(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - (1 - \sigma^2)^2 c^2}}
    \end{equation*}
    Plug in $\theta = 1- \sigma^2$, we get:
    \begin{equation*}
        \E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]
        = \frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}}
    \end{equation*}
    which finishes the proof.
\end{proof}

Now, we compute expectation over $x_u$ and $x_v$.

\begin{proposition}
\label{prop_singelSample}
The expected value of $\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]$ over $x_u$ and $x_v$ is
\begin{align}
\label{eq_singlesample}
\begin{split}
    \E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]
    = & \frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]
\end{split}
\end{align}
\end{proposition}

\begin{proof}
    There are 4 cases in the computation of expectation over $x_u$ and $x_v$:
    \begin{itemize}
        \item Case 1 ($x_u = x_v = 0$): we have $\frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}} = \frac{1}{\sqrt{1 - \theta^2 c^2}}$ and $P[\text{case 1}] = (1-\rho)^2$.
        \item Case 2 ($x_u = 0$, $x_v = \pm \frac{1}{\sqrt{\rho}}$ or $x_v = 0$, $x_u = \pm \frac{1}{\sqrt{\rho}}$): we have $\frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}} = \frac{\exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2})}{\sqrt{1 - \theta^2 c^2}}$ and $P[\text{case 2}] = 2 \rho (1-\rho)$.
        \item Case 3 ($x_u = x_v = \frac{1}{\sqrt{\rho}}$ or $x_u = x_v = -\frac{1}{\sqrt{\rho}}$): we have $\frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}} = \frac{\exp(\frac{c}{\rho (1 + \theta c)})}{\sqrt{1 - \theta^2 c^2}}$ and $P[\text{case 3}] = \frac{\rho^2}{2}$.
        \item Case 4 ($x_u = \frac{1}{\sqrt{\rho}}$, $x_v = -\frac{1}{\sqrt{\rho}}$ or $x_u = -\frac{1}{\sqrt{\rho}}$, $x_v = \frac{1}{\sqrt{\rho}}$): we have $\frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}} = \frac{\exp(-\frac{c}{\rho (1 - \theta c)})}{\sqrt{1 - \theta^2  c^2}}$ and $P[\text{case 4}] = \frac{\rho^2}{2}$.
    \end{itemize}
    Plug these into $\E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]$, we get:
    \begin{align*}
        \E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]]
        = & \E_{x_u, x_v}\Big [\frac{\exp \Paren{\frac{1}{2 - 2 \theta^2 c^2} [2 x_u x_v c - \theta(x_u^2 + x_v^2)c^2]}}{\sqrt{1 - \theta^2 c^2}} \Big] \\
        = & \frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
        & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]
    \end{align*}
\end{proof}

\subsection{Second Moment of Likelihood Ratio}

Given proposition \ref{prop_singelSample}, we can get the expression for $\E_{Z \sim \mu_0} [(L(Z))^2]$.
\begin{proposition}
Let $\theta = 1 - \sigma^2$ and $c = u^{\top} v$,
    \begin{align}
    \label{eq_likelihoodratioExact}
    \begin{split}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        = & \E_{c} \Big \{ \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
        & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n \Big \}
    \end{split}
    \end{align}
\end{proposition}

\begin{proof}
Plug equation \ref{eq_singlesample} into equation \ref{eq_multisample}, we get:
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \E_{u, v \sim S^{d-1}} [(\E_{x_u, x_v}[\E_{z \sim D_{\emptyset}}[\bar{D}_{u, x_u} (z) \cdot \bar{D}_{v, x_v} (z)]])^n] \\
    = & \E_{c} \Big \{ \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n \Big \}
\end{align*}
\end{proof}

In the following sections, we will first consider the case where $\sigma \rightarrow 0$, such that we have $\theta = 1 - \sigma^2 \rightarrow 1$ and:
\begin{align}
\label{eq_likelihoodratioLimit}
\begin{split}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \E_{c} \Big \{ \Big( \frac{1}{\sqrt{1 - c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{c^2}{2 - 2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1+c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1-c)}) \Big] \Big)^n \Big \}
\end{split}
\end{align}
Then, we will show that when $\sigma \leq d^{-K}$ for some constant $K$ that is large enough, we can bound equation \ref{eq_likelihoodratioExact} by equation \ref{eq_likelihoodratioLimit}. Notice that, in the noiseless model, we only consider the case where $c \neq \pm 1$ or $0$ because the probability measure of $c = \pm 1$ or $0$ is $0$ for $u, v$ sampled independently and uniformly at random from the unit sphere.

A key observation is that the random variable $y = \frac{c+1}{2}$ follows from Beta distribution with parameter $\alpha = \beta = \frac{d-1}{2}$, i.e. $y \sim Beta(\frac{d-1}{2}, \frac{d-1}{2})$. 

\begin{lemma}\label{lem:distribution-random-inner-product}
Let $u,v$ be two random $d$-dimensional vectors sampled uniformly from the unit sphere. Let $y = \frac{\iprod{u,v}+1}{2}$, 
    \begin{equation*}
        y \sim B(\frac{d-1}{2}, \frac{d-1}{2})
    \end{equation*}
\end{lemma}
We prove the lemma in appendix \ref{sec:probability-facts}. 

\begin{proposition}
    Let $y = \frac{c+1}{2}$ and $\sigma \rightarrow 0$,
    \begin{align}
    \label{eq_likelihoodratio}
    \begin{split}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        = & \Theta \Big \{ 2^{d-2} \sqrt{d-1} \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n [y(1-y)]^{\frac{d-3}{2}} dy \Big \}
    \end{split}
    \end{align}
\end{proposition}

\begin{proof}
     Apply change of variable by $c = 2y -1$ and take expectation over $y$,
    \begin{align*}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        = & \E_{y} \Big[\Big(\frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))]\Big)^n \Big] \\
        = & \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n P_y(y) dy
    \end{align*}
    Plug in the probability density function of $Beta(\frac{d-1}{2}, \frac{d-1}{2})$, we get:
    \begin{align*}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        = & \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n \frac{[y(1-y)]^{\frac{d-3}{2}}}{\cB(\frac{d-1}{2}, \frac{d-1}{2})} dy \\
        = & \frac{1}{\cB(\frac{d-1}{2}, \frac{d-1}{2})} \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n [y(1-y)]^{\frac{d-3}{2}} dy
    \end{align*}
    From Stirling's approximation, we get the following asymptotic bound for Beta function:
    \begin{equation}
    \label{eq_betaapprox}
        \cB(\frac{d-1}{2}, \frac{d-1}{2})
        = \Theta \Paren{\frac{((d-1)/2)^{d-2}}{(d-1)^{d-3/2}}}
        = \Theta \Paren{\frac{(1/2)^{d-2}}{\sqrt{d-1}}}
    \end{equation}
    Plug this into the likelihood ratio, we get:
    \begin{align*}
        \E_{Z \sim \mu_0} [(L(Z))^2]
        = & \Theta \Paren{2^{d-2} \sqrt{d-1}} \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n [y(1-y)]^{\frac{d-3}{2}} dy \\
        = & \Theta \Big \{ 2^{d-2} \sqrt{d-1} \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
        & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n [y(1-y)]^{\frac{d-3}{2}} dy \Big \}
    \end{align*}
\end{proof}

\subsection{Lower Bound for Rademacher Vectors}

We first discuss the case where $\rho = 1$, i.e. the planted vector $x$ is Rademacher, and prove that $\cP$ and $\cQ$ are statistically indistinguishable when the sample size $n \leq (1-\delta) d$ for some constant $\delta \in (0, 1)$.

\begin{theorem}
\label{theorem_nonSparseLikelihoodRatio}
Let $\rho = 1$ and $\sigma \rightarrow 0$. When $n \leq (1-\delta) d$ for some constant $\delta \in (0, 1)$,
\begin{equation*}
    E_{Z \sim \mu_0} [(L(Z))^2] \leq O(1)
\end{equation*}
\end{theorem}

\begin{proof}
When $\rho = 1$, equation \ref{eq_likelihoodratio} becomes:
\begin{equation*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = \Theta \Big\{2^{d-2-n} \sqrt{d-1} \int_{0}^{1} [y(1-y)]^{\frac{d-3-n}{2}} \Big( \frac{1}{2} \exp(1-\frac{1}{2 y}) + \frac{1}{2} \exp(1-\frac{1}{2 -  2 y})\Big)^n dy \Big\}
\end{equation*}
Notice that $\frac{1}{2} \exp(1-\frac{1}{2 y}) + \frac{1}{2} \exp(1-\frac{1}{2 -  2 y}) \leq 1$ on $y \in (0, 1)$, we have:
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \Theta \Big\{2^{d-2-n} \sqrt{d-1} \int_{0}^{1} [y(1-y)]^{\frac{d-3-n}{2}} \Big( \frac{1}{2} \exp(1-\frac{1}{2 y}) + \frac{1}{2} \exp(1-\frac{1}{2 -  2 y})\Big)^n dy \Big\} \\
    \leq & \Theta \Paren{2^{d-2-n} \sqrt{d-1} \int_{0}^{1} [y(1-y)]^{\frac{d-3-n}{2}} dy} \\
    = & \Theta \Paren{2^{d-2-n} \sqrt{d-1} \frac{\sqrt{\pi} 2^{-d+n+2} \Gamma((d-n-1)/2)}{\Gamma((d-n)/2)}} \\
    = & \Theta \Paren{\sqrt{d-1} \frac{\Gamma((d-n-1)/2)}{\Gamma((d-n)/2)}}
\end{align*}
Since $n \leq (1-\delta) d$ for some constant $\delta \in (0, 1)$, we have:
\begin{equation*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    \leq \Theta \Paren{\sqrt{d-1} \frac{\Gamma((\delta d-1)/2)}{\Gamma(\delta d/2)}}
\end{equation*}
From Stirling's approximation, we get the following asymptotic bound for Gamma function:
\begin{equation*}
    \Gamma(x+1)
    = \Theta \Paren{\sqrt{x} (\frac{x}{e})^x}
\end{equation*}
Therefore, we have $\Gamma(\frac{\delta d-1}{2}) = \Theta \Paren{\sqrt{\frac{\delta d - 3}{2}} (\frac{\delta d -3}{2e})^{\frac{\delta d -3}{2}}}$ and $\Gamma(\frac{\delta d}{2}) = \Theta \Paren{\sqrt{\frac{\delta d - 2}{2}} (\frac{\delta d -2}{2e})^{\frac{\delta d -2}{2}}}$. Now, we can get:
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \Theta \Paren{\sqrt{d-1} \frac{\Gamma((\delta d-1)/2)}{\Gamma(\delta d/2)}} \\
    = & \Theta \Paren{\sqrt{d-1} \frac{\sqrt{\frac{\delta d - 3}{2}} (\frac{\delta d -3}{2e})^{\frac{\delta d -3}{2}}}{\sqrt{\frac{\delta d - 2}{2}} (\frac{\delta d -2}{2e})^{\frac{\delta d -2}{2}}}} \\
    = & \Theta \Paren{\sqrt{\frac{d-1}{\delta d - 3}}} \\
    = & \Theta \Paren{\sqrt{\frac{1}{\delta}}}
\end{align*}
Since $\delta$ is a constant in $(0, 1)$, we have $\E_{Z \sim \mu_0} [(L(Z))^2] \leq O(1)$.
\end{proof}

\subsection{Lower Bounds for Sparse Rademacher Vectors when Noise $\sigma \rightarrow 0$}

Now, we prove that, when $\sigma \rightarrow 0$, we have lower bound $n \leq C_n \rho^2 d$ for $\rho$-sparse vectors with sparsity $\rho \geq \sqrt{\frac{\log d}{C_{\rho} d}}$ for some constant $C_n, C_{\rho} > 0$ that are small enough.

\begin{theorem}
\label{theorem_noiselessSparseLikelihoodRatio}
Let $\sigma \rightarrow 0$. When $n \leq C_n \rho^2 d$ and $\rho \geq \sqrt{\frac{\log d}{C_{\rho} d}}$ for some constant $C_n, C_{\rho} > 0$ that are small enough,
\begin{equation*}
    E_{Z \sim \mu_0} [(L(Z))^2] \leq O(1)
\end{equation*}
\end{theorem}

\begin{proof}
From equation \ref{eq_likelihoodratio}, we have:
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \Theta \Big\{2^{d-2} \sqrt{d-1} \int_{0}^{1} \Big( \frac{1}{2\sqrt{y(1-y)}} [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))] \Big)^n [y(1-y)]^{\frac{d-3}{2}} dy \Big\} \\
    = & \Theta \Big\{\sqrt{d-1} \int_{0}^{1} \Big((1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n [4y(1-y)]^{\frac{d-n-3}{2}} dy \Big\} \\
    = & \Theta \Big\{\sqrt{d-1} \int_{0}^{\frac{1}{2}} \Big((1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n [1-(2y-1)^2]^{\frac{d-n-3}{2}} dy \Big\} \\
    \leq & \Theta \Big\{\sqrt{d-1} \int_{0}^{\frac{1}{2}} \Big((1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \Big\}
\end{align*}
Notice that $\frac{(2y -1)^2}{y(1-y)} \geq 0$, which implies that $\exp(- \frac{1}{\rho} \frac{(2y -1)^2}{8y(1-y)}) \leq 1$ and
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    \leq & \Theta \Big\{\sqrt{d-1} \int_{0}^{\frac{1}{2}} \Big((1-\rho)^2 + 2 \rho (1-\rho) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \Big\} \\
    = & \Theta \Big\{\sqrt{d-1} \int_{0}^{\frac{1}{2}} \Big(1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \Big\}
\end{align*}
Now, we bound the integral by splitting it into two parts $[\frac{1}{2} - 0.001 \rho, \frac{1}{2}]$ and $(0, \frac{1}{2} - 0.001 \rho)$ such that:
\begin{align}
\label{eq_infolbsparse1}
\begin{split}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    \leq & \Theta \Big\{\sqrt{d-1} \int_{0}^{\frac{1}{2}} \Big(1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) \\
    & + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \Big\} \\
    = & \Theta \Big\{ P_1 + P_2 \Big \}
\end{split}
\end{align}
where
\begin{equation*}
    P_1 = 
    \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \Big(1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy
\end{equation*}
and,
\begin{equation*}
    P_2 = 
    \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} \Big(1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy
\end{equation*}

\subsubsection*{Bound $P_1$}

In this case, we have $y \in [\frac{1}{2} - 0.001 \rho, \frac{1}{2}]$, which implies that $0 \leq \frac{1}{\rho}(1-\frac{1}{2 -  2 y}) \leq 0.002$ and $-0.003 \leq \frac{1}{\rho}(1-\frac{1}{2 y}) \leq 0$. Note that the inequality $\exp(x) \leq 1 + x + x^2$ holds for $x \in [-1, 1]$. Therefore, we can apply this inequality to $\Delta = \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))$ and get:
\begin{align*}
    \Delta
    = & \frac{\rho^2}{2} \Big( \exp(\frac{1}{\rho}(1-\frac{1}{2 y})) + \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big) \\
    \leq & \frac{\rho^2}{2} \Big( 1 + \frac{1}{\rho}(1-\frac{1}{2 y}) + \frac{1}{\rho^2}(1-\frac{1}{2 y})^2 + 1 + \frac{1}{\rho}(1-\frac{1}{2-2 y}) + \frac{1}{\rho^2}(1-\frac{1}{2-2 y})^2 \Big) \\
    = & \frac{\rho^2}{2} \Big( 2 + \frac{1}{\rho}(2-\frac{1}{2 y} -\frac{1}{2-2 y}) + \frac{1}{\rho^2} [(\frac{2y - 1}{2 y})^2 + (\frac{2y-1}{2-2 y})^2] \Big) \\
    = & \frac{\rho^2}{2} \Big( 2 - \frac{1}{\rho} \frac{(2y-1)^2}{2y(1-y)} + \frac{(2y - 1)^2}{\rho^2} [(\frac{1}{2 y})^2 + (\frac{1}{2-2 y})^2] \Big) \\
    \leq & \frac{\rho^2}{2} \Big(2 + \frac{(2y - 1)^2}{\rho^2} [(\frac{1}{2 y})^2 + (\frac{1}{2-2 y})^2] \Big) \\
    = & \rho^2 + \frac{(2y - 1)^2}{2} [(\frac{1}{2 y})^2 + (\frac{1}{2-2 y})^2]
\end{align*}
Notice that $2 y \geq 1 - 0.002 \rho \geq 0.998$ and $2 - 2y \geq 1$, we have $(\frac{1}{2 y})^2 \leq (\frac{1}{0.998})^2$ and $(\frac{1}{2 - 2y})^2 \leq 1$. Let $c = \frac{1}{2} [(\frac{1}{0.998})^2 + 1]$, we get:
\begin{align*}
    \Delta
    \leq & \rho^2 + \frac{(2y - 1)^2}{2} [(\frac{1}{2 y})^2 + (\frac{1}{2-2 y})^2] \\
    \leq & \rho^2 + c (2y - 1)^2
\end{align*}
Plug this into $P_1$, we get:
\begin{align*}
    P_1
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \Big(1 - \rho^2 + \rho^2 + c (2y - 1)^2 \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    = & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \Big(1 + c (2y - 1)^2 \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big(c (2y - 1)^2 n \Big) \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big(c (2y - 1)^2 n - (2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big((2y - 1)^2 [- \frac{1}{2} + (c + \frac{1}{2}) \frac{n}{d} + \frac{3}{2d}] d \Big) dy
\end{align*}
Since we only consider $n \leq C_n \rho^2 d$ for some $C_n$ that is small enough and $d \rightarrow \infty$, we get:
\begin{equation*}
    - \frac{1}{2} + (c + \frac{1}{2}) \frac{n}{d} + \frac{3}{2d}
    \leq - \frac{1}{2} + (c + \frac{1}{2}) C_n \rho^2 + \frac{3}{2d}
    \leq - \frac{1}{2} + (c + \frac{1}{2}) C_n + \frac{3}{2d}
    \leq - c'
\end{equation*}
for some constant $c' > 0$.
Therefore, we have:
\begin{align*}
    P_1
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big((2y - 1)^2 [- \frac{1}{2} + (c + \frac{1}{2}) \frac{n}{d} + \frac{3}{2d}] d \Big) dy \\
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big(- c' (2y - 1)^2 d \Big) dy
\end{align*}
Apply change of variables to the integral by $w = (2y-1)\sqrt{c' d}$, we get:
\begin{align*}
    P_1
    \leq & \sqrt{d-1} \int_{\frac{1}{2} - 0.001 \rho}^{\frac{1}{2}} \exp \Big(- c' (2y - 1)^2 d \Big) dy \\
    \leq &  \frac{\sqrt{d-1}}{2 \sqrt{c' d}} \int_{- 0.002 \rho \sqrt{c' d}}^{0} \exp (- w^2) dw \\
    \leq &  \frac{\sqrt{d-1}}{2 \sqrt{c' d}} \int_{- \infty}^{ \infty } \exp (- w^2) dw \\
    = & \frac{\sqrt{\pi (d-1)}}{2 \sqrt{c' d}} \\
    = & O(1)
\end{align*}

\subsubsection*{Bound $P_2$}

In this case, we have $y \in (0, \frac{1}{2} - 0.001 \rho)$, which implies $1 - \frac{1}{2y} \leq 0$ and $\exp(\frac{1}{\rho}(1-\frac{1}{2 y})) \leq 1$. Therefore, we have:
\begin{align*}
    P_2
    \leq & \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} \Big(1 - \rho^2 + \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    = & \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} \Big(1 - \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) dy \\
    = & \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} h(y) dy
\end{align*}
where $h(y) = \Big(1 - \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big)$. Now, we will prove that for any $y \in (0, \frac{1}{2} - 0.001 \rho)$, we have:
\begin{equation*}
    h(y) \leq \exp(- \log d)
\end{equation*}
We prove this by showing that this inequality holds for both case (1): $1 - \frac{\rho^2}{2} \leq \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))$ and case (2): $1 - \frac{\rho^2}{2} \geq \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))$.

\paragraph*{Case (1)}  In this case, we have $1 - \frac{\rho^2}{2} \leq \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))$ and
\begin{align*}
    h(y)
    = & \Big(1 - \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & \Big(\rho^2 \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    = & \rho^{2n} \exp \Big(\frac{n}{\rho}(1-\frac{1}{2 -  2 y}) - (2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & \exp \Big( (1-2y) \Big[\frac{n}{\rho(2 -  2 y)} - (1-2y) \frac{d-n-3}{2} \Big] \Big) \\
    \leq & \exp \Big( (1-2y) \Big[\frac{n}{\rho} - 0.001 \rho (d-n-3) \Big] \Big) \\
    \leq & \exp \Big( (1-2y) \Big[- 0.001 \rho d + (0.001 \rho + \frac{1}{\rho}) n + 0.003 \rho \Big] \Big)
\end{align*}
Since we only consider $n \leq C_n \rho^2 d$ for some $C_n$ that is small enough and $d \rightarrow \infty$, we get:
\begin{align*}
    h(y)
    \leq & \exp \Big( (1-2y) \Big[- 0.001 \rho d + (0.001 \rho + \frac{1}{\rho}) n + 0.003 \rho \Big] \Big) \\
    \leq & \exp \Big( (1-2y) \Big[- 0.001 \rho d + (0.001 \rho + \frac{1}{\rho}) C_n \rho^2 d + 0.003 \rho \Big] \Big) \\
    = & \exp \Big( (1-2y) \Big[(- 0.001 + C_n) \rho d + 0.001 C_n \rho^3 d + 0.003 \rho \Big] \Big) \\
    \leq & \exp \Big( 0.002 \rho \Big[(- 0.001 + C_n) \rho d + 0.001 C_n \rho^3 d + 0.003 \rho \Big] \Big) \\
    \leq & \exp \Big(- c'' \rho^2 d \Big)
\end{align*}
for some constant $c'' > 0$. Since $\rho \geq \sqrt{\frac{\log d}{C_{\rho} d}}$, we have $- c'' \rho^2 d \leq - \frac{c'' \log d}{C_{\rho}} \leq - \log d$ for some positive constant $C_{\rho}$ that is small enough. Hence, in case (1), we have:
\begin{equation*}
    h(y)
    \leq \exp \Big(- c'' \rho^2 d \Big)
    \leq \exp(- \log d)
\end{equation*}

\paragraph*{Case (2)} In this case, we have $1 - \frac{\rho^2}{2} \geq \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y}))$ and
\begin{align*}
    h(y)
    = & \Big(1 - \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}(1-\frac{1}{2 -  2 y})) \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & \Big(2 - \rho^2 \Big)^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & 2^n \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & \exp(n) \exp \Big(-(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    = & \exp \Big(n -(2y-1)^2 \frac{d-n-3}{2} \Big) \\
    \leq & \exp \Big(n - 0.00002 \rho^2 (d-n-3) \Big) \\
    = & \exp \Big( - 0.00002 \rho^2 d + n + 0.00002 \rho^2  n + 0.00006 \rho^2  \Big)
\end{align*}
Since we only consider $n \leq C_n \rho^2 d$ for some $C_n$ that is small enough and $d \rightarrow \infty$, we get:
\begin{align*}
    h(y)
    \leq & \exp \Big( - 0.00002 \rho^2 d + n + 0.00002 \rho^2  n + 0.00006 \rho^2  \Big) \\
    \leq & \exp \Big( - 0.00002 \rho^2 d + C_n \rho^2 d + 0.00002 C_n \rho^4 d + 0.00006 \rho^2  \Big) \\
    \leq & \exp \Big( - c''' \rho^2 d \Big)
\end{align*}
for some constant $c''' > 0$. Since $\rho \geq \sqrt{\frac{\log d}{C_{\rho} d}}$, we have $- c''' \rho^2 d \leq - \frac{c''' \log d}{C_{\rho}} \leq - \log d$ for some positive constant $C_{\rho}$ that is small enough. Hence, in case (2), we have:
\begin{equation*}
    h(y)
    \leq \exp \Big(- c''' \rho^2 d \Big)
    \leq \exp(- \log d)
\end{equation*}

Combine case (1) and case (2), we can conclude that the following holds for arbitrary $y \in (0, \frac{1}{2} - 0.001 \rho)$:
\begin{equation*}
    h(y) \leq \exp(- \log d)
\end{equation*}
Plug this into $P_2$, we get:
\begin{align*}
    P_2
    \leq & \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} h(y) dy \\
    \leq & \sqrt{d-1} \int_{0}^{\frac{1}{2} - 0.001 \rho} \exp(- \log d) dy \\
    \leq & \sqrt{d-1} \exp(- \log d) \\
    = & \frac{\sqrt{d-1}}{d} \\
    = & O(1)
\end{align*}

\subsubsection*{Combine $P_1$ and $P_2$}

Now, we have shown that $P_1 \leq O(1)$ and $P_2 \leq O(1)$. Plug these into equation \ref{eq_infolbsparse1}, we get:
\begin{equation*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    \leq \Theta \Big\{ P_1 + P_2 \Big \}
    \leq O(1)
\end{equation*}

\end{proof}

\subsection{Lower Bound for Noisy Sparse Rademacher Vectors}

\begin{theorem}
\label{theorem_noisySparseLikelihoodRatio}
Let $\sigma \leq d^{-K}$ for some constant $K$ that is large enough and $\theta = 1 - \sigma^2$. When $n \leq C_n \rho^2 d$ and $\rho \geq \sqrt{\frac{\log d}{C_{\rho} d}}$ for some constant $C_n, C_{\rho} > 0$ that are small enough,
\begin{equation*}
    E_{Z \sim \mu_0} [(L(Z))^2] \leq O(1)
\end{equation*}
\end{theorem}

\begin{proof}
From equation \ref{eq_likelihoodratioExact}, we can get:
\begin{align*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    = & \E_{c} \Big \{ \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n \Big \} \\
    = & \int_{-1}^{1} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc \\
    = & 2 \int_{0}^{1} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc \\
    = & 2 \Big \{ Q_1 + Q_2 \Big \}
\end{align*}
where
\begin{align*}
    Q_1 = & \int_{0}^{1-d^{-k}} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc
\end{align*}
and
\begin{align*}
    Q_2 = & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc
\end{align*}
for some constant $k$ that is large enough but smaller than $\frac{K}{2}$.

\subsubsection*{Bound $Q_1$}

Notice that, for $0 \leq c \leq 1-d^{-k}$, we have:
\begin{align}
\label{eq_infoNoisySparseVector1}
\begin{split}
    \frac{\exp(\frac{c}{\rho (1 + \theta c)})}{\exp(\frac{c}{\rho (1 + c)})}
    & = \exp(\frac{c}{\rho (1 + \theta c)} - \frac{c}{\rho (1 + c)}) \\
    & = \exp(\frac{c^2 (1 - \theta)}{\rho (1 + \theta c) (1 + c)})\\
    & = \exp(\frac{c^2 \sigma^2}{\rho (1 + \theta c) (1 + c)})\\
    & \leq \exp(\frac{4 \sigma^2}{\rho})
\end{split}
\end{align}
and,
\begin{align}
\label{eq_infoNoisySparseVector2}
\begin{split}
    \frac{\exp(- \frac{c}{\rho (1 - \theta c)})}{\exp(- \frac{c}{\rho (1 - c)})}
    & = \exp(\frac{-c}{\rho (1 - \theta c)} - \frac{-c}{\rho (1 - c)}) \\
    & = \exp(\frac{c^2 (1 - \theta)}{\rho (1 - \theta c) (1 - c)})\\
    & = \exp(\frac{c^2 \sigma^2}{\rho (1 - \theta c) (1 - c)})\\
    & \leq \exp(\frac{4 \sigma^2}{\rho d^{-2k}})
\end{split}
\end{align}
where we used $1 - \theta c \geq 1 - c \geq d^{-k}$ in the last step. Since $\rho \geq d^{-1/2}$ and $\sigma \leq d^{-K}$, we have $\frac{4 \sigma^2}{\rho} \leq d^{-2K + 1}$ and $\frac{4 \sigma^2}{\rho d^{-2k}} \leq d^{-2K + 2k + 1}$. Let $k' = 2K - 2k - 1$, we have $k' > K-1$, $\frac{4 \sigma^2}{\rho} \leq d^{-2K + 1} \leq d^{-k'}$ and $\frac{4 \sigma^2}{\rho d^{-2k}} \leq d^{-k'}$. Therefore, we can get:
\begin{equation*}
    \exp(\frac{c}{\rho (1 + \theta c)})
    \leq \exp(\frac{4 \sigma^2}{\rho}) \exp(\frac{c}{\rho (1 + c)})
    \leq \exp(d^{-k'}) \exp(\frac{c}{\rho (1 + c)})
\end{equation*}
and
\begin{equation*}
    \exp(- \frac{c}{\rho (1 - \theta c)})
    \leq \exp(\frac{4 \sigma^2}{\rho d^{-2k}}) \exp(- \frac{c}{\rho (1 - c)})
    \leq \exp(d^{-k'}) \exp(- \frac{c}{\rho (1 - c)})
\end{equation*}
Plug this into $Q_1$, we get:
\begin{align*}
    Q_1
    = & \int_{0}^{1-d^{-k}} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc \\
    \leq & \int_{0}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [1 - \rho^2 + \exp(d^{-k'}) \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + c)}) + \exp(d^{-k'}) \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - c)}) \Big]\Big)^n P(c) dc \\
    \leq & \int_{0}^{1} \Big(\exp(d^{-k'}) \frac{1}{\sqrt{1 - c^2}} \Big [1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - c)}) \Big]\Big)^n P(c) dc \\
    = & \exp(n d^{-k'})\int_{0}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - c)}) \Big]\Big)^n P(c) dc
\end{align*}
Notice that $\exp(n d^{-k'}) < \exp(d^{-k'+1}) < \exp(1)$ and $\int_{0}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [1 - \rho^2 + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - c)}) \Big]\Big)^n P(c) dc$ can be bounded by $P_1 + P_2$ as defined in equation \ref{eq_infolbsparse1}, we have:
\begin{equation*}
    Q_1 \leq \exp(1) (P_1 + P_2) \leq O(1)
\end{equation*}

\subsubsection*{Bound $Q_2$}

When $1-d^{-k} \leq c \leq 1$, we have $- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2} \leq 0$, $\frac{c}{\rho (1 + \theta c)} \leq \frac{1}{\rho}$ and $-\frac{c}{\rho (1 - \theta c)} \leq 0$, which implies:
\begin{align*}
    Q_2
    = & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - \theta^2 c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) \exp(- \frac{1}{\rho} \frac{\theta c^2}{2 - 2 \theta^2 c^2}) \\
    & + \frac{\rho^2}{2} \exp(\frac{c}{\rho (1 + \theta c)}) + \frac{\rho^2}{2} \exp(-\frac{c}{\rho (1 - \theta c)}) \Big]\Big)^n P(c) dc \\
    \leq & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [(1-\rho)^2 + 2 \rho (1-\rho) + \frac{\rho^2}{2} \exp(\frac{1}{\rho}) + \frac{\rho^2}{2} \Big]\Big)^n P(c) dc \\
    = & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [1 - \frac{\rho^2}{2} + \frac{\rho^2}{2} \exp(\frac{1}{\rho}) \Big]\Big)^n P(c) dc \\
    \leq & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \Big [1 + \frac{1}{2} \exp(\frac{1}{\rho}) \Big]\Big)^n P(c) dc
\end{align*}
Since we have $\frac{1}{2} \exp(\frac{1}{\rho}) \geq 1$ for $\rho \leq 1$, we can get:
\begin{align*}
    Q_2
    \leq & \int_{1-d^{-k}}^{1} \Big(\frac{1}{\sqrt{1 - c^2}} \exp(\frac{1}{\rho}) \Big)^n P(c) dc \\
    \leq & \int_{1-d^{-k}}^{1} \frac{1}{(\sqrt{1 - c^2})^n}  \exp \Big(\frac{n}{\rho} \Big) P(c) dc \\
    = & \exp \Big(\frac{n}{\rho} \Big) \int_{1-d^{-k}}^{1} \frac{1}{(\sqrt{1 - c^2})^n} P(c) dc
\end{align*}
Plug in $n \leq C_n \rho^2 d$, we get:
\begin{align*}
    Q_2
    \leq & \exp (C_n \rho d) \int_{1-d^{-k}}^{1} \frac{1}{(\sqrt{1 - c^2})^n} P(c) dc \\
    \leq & \exp (C_n d) \int_{1-d^{-k}}^{1} \frac{1}{(\sqrt{1 - c^2})^n} P(c) dc
\end{align*}
Now, we plug in $c = 2y - 1$ and $y \sim Beta(\frac{d-1}{2}, \frac{d-1}{2})$:
\begin{align*}
    Q_2
    \leq & \exp (C_n d) \int_{1-d^{-k}}^{1} \frac{1}{(\sqrt{1 - (2y-1)^2})^n} P(y) dy \\
    = & \exp (C_n d) \int_{1-d^{-k}/2}^{1} \frac{1}{(\sqrt{4y-4y^2})^n} \frac{[y(1-y)]^{\frac{d-3}{2}}}{\cB(\frac{d-1}{2}, \frac{d-1}{2})} dy \\
    = & \Theta \Big \{ \exp (C_n d) \int_{1-d^{-k}/2}^{1} 2^{d-n} \sqrt{d-1} [y(1-y)]^{\frac{d-n-3}{2}} dy \Big \}
\end{align*}
Since $1 - \frac{d^{-k}}{2} \leq y \leq 1$ and $0 \leq 1 - y \leq \frac{d^{-k}}{2}$, we have:
\begin{align*}
    Q_2
    \leq & \Theta \Big \{ \exp (C_n d) \int_{1-d^{-k}/2}^{1} 2^{d-n} \sqrt{d-1} \Big (\frac{d^{-k}}{2} \Big)^{\frac{d-n-3}{2}} dy \Big \} \\
    = & \Theta \Big \{ \exp (C_n d) \int_{1-d^{-k}/2}^{1} 2^{(d-n)/2} \sqrt{d-1} d^{\frac{-k(d-n-3)}{2}} dy \Big \} \\
    = & \Theta \Big \{ \exp (C_n d ) \frac{d^{-k}}{2} 2^{(d-n)/2} \sqrt{d-1} d^{\frac{-k(d-n-3)}{2}} \Big \} \\
    \leq & \Theta \Big \{ \exp (C_n d) \exp(d) d^{ - \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}} \Big \} \\
    \leq & \Theta \Big \{ \exp (C_n d + d) d^{ - \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}} \Big \}
\end{align*}
Now, consider $- \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}$, plug in $n \leq C_n \rho^2 d$, we get:
\begin{equation*}
    - \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}
    \leq - \frac{kd}{2} + \frac{k C_n \rho^2 d}{2} + \frac{k}{2} + \frac{1}{2}
    = - (1 - C_n \rho^2) \frac{k}{2} d + \frac{k}{2} + \frac{1}{2}
\end{equation*}
Since $C_n \rho^2 < 1$, there exists a constant $0 < k'' < (1 - C_n \rho^2)\frac{k}{2}$ such that:
\begin{equation*}
    - \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}
    \leq - (1 - C_n \rho^2) \frac{k}{2} d + \frac{k}{2} + \frac{1}{2}
    \leq - k'' d
\end{equation*}
Hence, we have:
\begin{align*}
    Q_2
    \leq & \Theta \Big \{ \exp (C_n d + d) d^{ - \frac{kd}{2} + \frac{kn}{2} + \frac{k}{2} + \frac{1}{2}} \Big \} \\
    \leq & \Theta \Big \{ \exp (C_n d + d) d^{ - k''d} \Big \} \\
    \leq & \Theta \Big \{ \exp (C_n d + d -k'' d \log d) \Big \} \\
    \leq & O(1)
\end{align*}

\subsubsection*{Combine $Q_1$ and $Q_2$}

Combine $Q_1$ and $Q_2$, we get:
\begin{equation*}
    \E_{Z \sim \mu_0} [(L(Z))^2]
    \leq 2 \Big \{ Q_1 + Q_2 \Big \}
    \leq O(1)
\end{equation*}
when $\sigma \leq d^{-K}$ for some constant $K$ that is large enough.

\end{proof}


==> content/Techniques.tex <==
\section{Background and prior work}

\subsection{Failure of SQ lower bound}
Although the majority of machine learning algorithms are captured by SQ algorithm, Gaussian elimination and its alike can surpass SQ lower bound. A celebrated scenario for the failure of SQ lower bound is learning parity function \cite{Blum2003NoisetolerantLT}.
 It is worth mentioning that, very recently, the SQ lower bound was also found to fall short in asymmetric tensor PCA model \cite{Dudeja2021StatisticalQL}.  

\subsection{Algorithm results for Sparse Planted Vector problem}
For the Random Sparse Planted Vector problem we consider here, it has been shown that the $l_1 / l_2$ minimization problem recovers the planted vector as long as $\rho \leq c$ and $d \leq cn$ for a sufficiently small constant $c$ \cite{qu2014finding}. However, the $l_1 / l_2$ minimization problem is non-convex and is computationally expensive. The sum-of-squares method proposed in \cite{barak2014rounding} estimates the planted vector based on the $l_2 / l_4$ minimization problem in the region $\rho \leq c$ and $d \sqrt{\rho} \leq c \sqrt{n}$. Inspired by the sum-of-squares method, a fast spectral method to estimate the planted vector was proposed in \cite{hopkins2016fast} which works in the region $\rho \leq c$ and $d \ll \sqrt{n}$. The optimal spectral algorithm was proposed in \cite{mao2021optimal} which builds on \cite{hopkins2016fast} and recovers the planted vector when $n \geq \tilde{\Omega}\Paren{\rho^2 d^2}$. Very surprisingly, it was recently shown in \cite{LLLalgorithm, KaneLLL} that Lattice based algorithms can recover the planted sparse vector when $n\geq \Omega(d)$, which surpasses previous lower bound on low degree polynomials. 
 
 \subsection{Computational lower bounds}
 For the Random Sparse Planted Vector problem, it was shown in \cite{mao2021optimal} that low-degree polynomial algorithms fail when $n \leq \tilde{O}\Paren{\rho^2 d^2}$. When the sparsity $\rho=1$, i.e. the planted vector is Rademacher, Sum of Squares lower bound is proved for $n\ll d^{3/2}$
 in \cite{ArbitraryNonSphericalGaussian}. These lower bounds are surpassed by the aforementioned lattice based algorithm in \cite{LLLalgorithm}. 
 
 \subsection{Relation to non-Gaussian component analysis}
The Random Sparse Planted Vector problem can be considered as a special case of non-Gaussian component analysis. In such class of models, conditioning on a hidden direction $u\in \mathbb{R}^d$, the samples $z_1,z_2,\ldots,z_n$ are i.i.d randomly distributed $d$-dimensional vectors. The projection of $z_i$ in the direction perpendicular to $u$  follows standard Gaussian distribution, while $\iprod{z_i,u}$ follows some specified non-Gaussian distribution. The problem is to estimate the hidden direction $u$.

Another famous Non-Gaussian component analysis model is homogeneous continuous learning with error (hCLWE) \cite{CLWE}. There are SQ lower bounds for this model when  inverse polynomial amount of Gaussian noise is added to the hidden direction \cite{parallelPancake,diakonikolas2017statistical}. However, note that the Lattice basis reduction algorithms are not believed to be robust against inverse polynomial amount of noise \cite{LLLalgorithm,KaneLLL}. Therefore, we cannot conclude that the LLL algorithm surpasses SQ lower bound in their setting.

